ChatGLM-Math: Improving Math Problem-Solving in Large Language Models with a Self-Critique Pipeline

Large language models (LLMs) have shown excellent mastering of human language, but still struggle in real-world applications that require mathematical problem-solving. While many strategies and datasets to enhance LLMs' mathematics are developed, it remains a challenge to simultaneously maintain and improve both language and mathematical capabilities in deployed LLM systems.In this work, we tailor the Self-Critique pipeline, which addresses the challenge in the feedback learning stage of LLM alignment. We first train a general Math-Critique model from the LLM itself to provide feedback signals. Then, we sequentially employ rejective fine-tuning and direct preference optimization over the LLM's own generations for data collection. Based on ChatGLM3-32B, we conduct a series of experiments on both academic and our newly created challenging dataset, MathUserEval. Results show that our pipeline significantly enhances the LLM's mathematical problem-solving while still improving its language ability, outperforming LLMs that could be two times larger. Related techniques have been deployed to ChatGLM\footnote{\url{https://chatglm.cn}}, an online serving LLM. Related evaluation dataset and scripts are released at \url{https://github.com/THUDM/ChatGLM-Math}.

==> table/alignbench.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Results of Alignbench~\cite{liu2023alignbench}, Language Part. \textmd{}}
\label{table:alignbench}
\begin{tabular}{@{}lc@{}}
\toprule
\multirow{2}{*}{Model}        & Language \\ \cmidrule(l){2-2} 
                              & AVG      \\ \midrule
gpt-4-1106-preview            & 8.29     \\
\textbf{GLM-Math-32b w/ DPO}  & 7.80     \\
gpt-4-0613                    & 7.59     \\
\textbf{GLM-Math-32b w/o DPO} & 7.43     \\
\textbf{GLM-32b}              & 7.38     \\
qwen-72b-chat                 & 7.29     \\
erniebot-3.5                  & 7.13     \\
DeepSeek-67B-Chat             & 7.11     \\
gpt-3.5-turbo-0613            & 6.82     \\
claude-2                      & 6.78     \\
yi-34b-chat                   & 6.18     \\ \bottomrule
\end{tabular}


\end{table}

==> table/first_table.tex <==

\begin{table}[t]
\caption{Our self-critique pipeline enables simultaneous improvement of language and mathematical abilities. Previously, alignment methods (such as DPO) enhance language but could potentially impair mathematical abilities~\cite{deepseekai2024deepseek}, whereas math-specialized models could harm language capabilities~\cite{2023internlm}. }
%\vspace{-3mm}
\label{tab:first table}
\centering
\footnotesize
%\centering
%\resizebox{\columnwidth}{!}{
\renewcommand\tabcolsep{.5pt}
%\renewcommand\arraystretch{1.1}
\vspace{1mm}
\begin{tabular}{@{}lcc@{}}

\toprule
Model & Avg. of GSM\&MATH & Language \\
\midrule
DeepSeek-67B-Chat~\cite{deepseekai2024deepseek} & 58.3 & 7.11 \\
DeepSeek-67B-Chat-DPO~\cite{deepseekai2024deepseek} & 57.7(\textbf{\textcolor{red}{-1.2\%}}) & 7.60(\textbf{\textcolor{teal}{+6.8\%}}) \\
\midrule
InternLM2-Chat-20B~\cite{2023internlm} & 57.2 & 7.68 \\
Math-InternLM2-20B~\cite{2023internlm} & 60.2(\textbf{\textcolor{teal}{+5.1\%}}) & 6.53(\textbf{\textcolor{red}{-14.8\%}}) \\
\midrule
ChatGLM3-32B-SFT & 52.4 & 7.37 \\
ChatGLM3-32B-SFT + RFT\&DPO & 61.6(\textbf{\textcolor{teal}{+17.5\%}}) & 7.80(\textbf{\textcolor{teal}{+5.85\%}}) \\
\bottomrule
\end{tabular}
% \vspace{-8mm}
\end{table}
